On Training and Evaluation of Neural Network Approaches for Model Predictive Control

The contribution of this paper is a framework for training and evaluation of Model Predictive Control (MPC) implemented using constrained neural networks. Recent studies have proposed to use neural networks with differentiable convex optimization layers to implement model predictive controllers. The motivation is to replace real-time optimization in safety critical feedback control systems with learnt mappings in the form of neural networks with optimization layers. Such mappings take as the input the state vector and predict the control law as the output. The learning takes place using training data generated from off-line MPC simulations. However, a general framework for characterization of learning approaches in terms of both model validation and efficient training data generation is lacking in literature. In this paper, we take the first steps towards developing such a coherent framework. We discuss how the learning problem has similarities with system identification, in particular input design, model structure selection and model validation. We consider the study of neural network architectures in PyTorch with the explicit MPC constraints implemented as a differentiable optimization layer using CVXPY. We propose an efficient approach of generating MPC input samples subject to the MPC model constraints using a hit-and-run sampler. The corresponding true outputs are generated by solving the MPC offline using OSOP. We propose different metrics to validate the resulting approaches. Our study further aims to explore the advantages of incorporating domain knowledge into the network structure from a training and evaluation perspective. Different model structures are numerically tested using the proposed framework in order to obtain more insights in the properties of constrained neural networks based MPC.

==> CDC 2020 MPC-NET/problem.tex <==
{\color{black}As discussed in the Section \ref{Sec1}, the goal of any learning approach to solving MPC problems is to obtain a meaningful mapping $\mu(\mathbf{x})$
such that for any given initial state $\mathbf{x}$, it produces the control law
\begin{equation*}
    \mathbf{u}=\mu(\mathbf{x}),
\end{equation*}
where $\mathbf{u}$ is the solution to the MPC. In order for one to make a consistent characterization of any learning approach, two important aspects have to be analyzed:
\begin{itemize}
    \item The nature of the mapping,
    \item The nature of data, in the context of training and evaluation.
\end{itemize}
Though learning approaches to MPC are not new, a framework for such a characterization of learning approaches in the MPC setting does not exist in literature.  
This motivates our present contribution in the form of a framework addressing these aspects, particularly in terms of training and evaluation through numerical experiments. We discuss these two aspects in detail next.

\subsection{The nature of $\mu(\mathbf{x})$}
Depending on the horizon, the state and input constraints, and the strategy employed, we have the following common variants of the MPC problem in general:
\begin{itemize}
    \item LQR, which corresponds to the unconstrained version of the infinite horizon problem \eqref{eq:constrained_infinite_horizon} ,
    
    \item Finite or infinite horizon control with constraints on the input and state vectors,
    
    \item Explicit MPC, which is a reformulation of the constrained MPC in terms of control invariant sets, giving a pre-computed offline lookup table-like characterization of the control law in terms of the state vector \cite{empc_bemporad},
    
    \item Learning based MPC approaches, which uses supervised learning from seen data examples typically in the form of a neural networks.
\end{itemize}
Correspondingly, each of these variants produce their own mapping $\mu(\mathbf{x})$. 
In the case of quadratic program based approaches for constrained MPC, $\mu(\mathbf{x})$ is obtained  by solving quadratic programs through convex optimization solvers such as the OSQP \cite{OSQP}. 

\subsection{The nature of data: Data generation for training and evaluation of $\mu(\mathbf{x})$}
Another key aspect in characterizing a learnt mapping is its relation to the available data-set. In terms of the training, this entails how the input space must be sampled such that the learning is meaningful and generalizes well. This aspect is of importance given that in many real-life applications such as vehicle control, one cannot be expected to have access to an unlimited number of diverse training data-points. 

In the case of the simple LQR,
$$
\mathbf{u}=-\mathbf{Lx}
$$
this poses no real difficulty since all that is needed to find $\mathbf{L}$ from training data is a single set of $n$ linearly independent samples of $x$ and corresponding $u$.

In the case of the explicit MPC, it comes with added complexity that one has to sample a set $n$ linearly independent points in each of the regions where the control law is constant.  For $q$ regions we thus need at least $n\times q$ samples of $\mathbf{x}$ and the corresponding $\mathbf{u}$.

Naturally, this issue also extends to the case where one wishes to work with neural network based learnt mappings -- how must we span the training space? One intuitively reasonable approach is that we uniformly sample the feasible set. To this end, we propose the use of a Hit-and-Run sampler which performs a random walk across the feasible set. In Figure \ref{fig:har_1000} we plot a set of 1000 points sampled using the hit-and-run sampler from the set $\mathcal{C}_{\infty}$ in Figure, \ref{fig:exA_cinf}. 
 The algorithm is presented in Section \ref{Sec5}.

We believe that this gives a consistent way of approaching the training aspect. Another related question, which we are currently pursuing, is whether it is more meaningful to incorporate the temporal aspect actively into the training process: rather than being randomly sampled isolated training data-points $\{\mathbf{x},\mathbf{u}\}$, should the training samples be from full trajectories?

The idea of representing a MPC with a structured neural network is also closely connected to the classical problem of function estimation from experimental data. This subject has a long history going back to the work of Box and co-workers on response surfaces \cite{Box}.  Gaussian processes and Bayesian optimization provide solid statistical frameworks for estimation of  function  and corresponding input design \cite{7352306}. Samples are typically chosen by optimizing a so-called acquisition function, which measures the current uncertainty of the function estimate. A simple method is  uncertainty sampling, where the next sample is taken where the uncertainty is the highest.  Unfortunately, less is understood regarding  optimal input design for the training of neural networks. %Since there is no explicit uncertainty in the data, we have a pure approximation problem.  
To obtain  insight into the approximation properties and generalization ability, we need tools to analyze the error and at the same time get information where to sample new data.
 Let $u=n(\mathbf{x})$ denote the network approximation of the MPC $\mathbf{u}=\mu(\mathbf{x})|$. On the training data we can calculate maximal error as
$\max_{\mathbf{x}_i\in\mathcal{D}}|n(\mathbf{x}_i)- \mu(\mathbf{x}_i)|$. 
Provided that the network is flexible enough these errors should be small after training. The challenge is to estimate the error for  $\mathbf{x}$ outside the sample set, and then sample additional  $\mathbf{x}$ where the errors are large. Recall that we also can calculate gradients with respect to $\mathbf{x}$ , i.e. $\nabla n(\mathbf{x})$ and  $\nabla d(\mathbf{x})$. Sub-gradients can be used  where the mappings are non-differentiable.
The gradient calculations can be done using CVXPY as described in \cite{agrawal2019differentiable}.
We then obtain information about the approximation error in a neighborhood around interesting sample points by computing the first order approximation
\begin{align*}
[n(\mathbf{x})- \mu(\mathbf{x})]&\approx  [n(\mathbf{x}_i)- \mu(\mathbf{x}_i)]\nonumber\\
&+ [\nabla n(\mathbf{x}_i)- \nabla n(\mathbf{x}_i)]^T(\mathbf{x}-\mathbf{x}_i)
\end{align*}
in a neighbourhood $||\mathbf{x}-\mathbf{x}_i||\leq \epsilon$ that does not overlap other existing samples of $\mathbf{x}$.
In order to generate new training data, we would like to identify regions where the approximation error is large. One way is to solve the QP
\begin{align*}
&\max_{\mathbf{x}}|| [\nabla n(\mathbf{x}_i)- \nabla d(\mathbf{x}_i)]^T(\mathbf{x}-\mathbf{x}_i)|| \nonumber\\ &\mbox{subject to}\;   ||\mathbf{x}-\mathbf{x}_i||\leq \epsilon
\end{align*}
for selected  $\mathbf{x}_i$ to obtain a measure where  to take new samples. 
 
Thus we see that it is possible to develop a well-motivated and systematic framework for the analysis and evaluation of learning based MPC. Our current contribution is a step in this direction.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{plots/exA_har_1000_samples.png}
    \caption{Hit-and-run sampling of 1000 points from the set $\mathcal{C}_{\infty}$ in Figure \ref{fig:exA_cinf}.}
    \label{fig:har_1000}
\end{figure}

}






==> CDC 2020 MPC-NET/story.tex <==
STORY LINE

 

We consider MPC of linear systems with linear constraint and quadratic cost function …

 

Questions: Use notation from the OSQP paper or the book? I suggest the OSQP notation

 

We use the standard MPC theory for feasibility and stability, ref book by Bemporad & co

 

We use OSQP for solving the MPC  to generate training data.

 

Why is it a good idea to store the solution for all x rather than running real time optimization? The vehicle industry is used to look up table control  and it is easy to evaluate/certify  by massive simulations

 

 

We have to understand  how the MPC control law u=\mu(x) looks like as a function of x

 

In order of simplicity

 

·       LQR u=-Lx

·       LQR with projection on the constraints

·       Explicit MPC

·       QP with linear constraints, take from OSQP paper that the solution for fixed active sets given by a set of linear equations. It is even more clear from the attached book chapter main.pdf (section 2.2). The challenge is that the active constraints are changing as a function of $x$ ( explicit MPC).

·       We can calculate the gradient of \mu(x) w.r.t. x using CVXPY: We expect the gradient to be constant in area where the control law is linear, and jump when we move between active constraint. Nice with a plot for the 2 state example. Plot mu(x) its derivative from dense gridding.

 

We have to understand  data generation for u=\mu(x), i.e. how should we sample x to obtain “optimal” information about the function =\mu(x) to be used for supervised learning?

 

·       LQR is easy. Just pick n linearly independent values of x and solve a linear equation

·       Explicit MPC is more difficult: Pick n linearly independent values of x in each subset where the control law is constant and solve  linear equations

·       Random sampling using hit and run. This is a good idea for covering a higher dimension set by random sampling

·       Should we use trajectories or not to for learning data?

·       Supervised sampling  where one needs new samples of where the fit is bad. Here we may use ideas from Gaussian Processes etc as I wrote

 

 

Given all this information other authors has proposed to use NN with ReLU and projection layers.

 

·       We have combined PyTorch and CVXPY to an easy environment for training and evaluation

·       There are guidelines in how many layers one needs for a given state dimension

·       There are some evidence that the projection layers are need, but we are not sure

·       How do we evaluate the learned NN? Here we propose  to measure the fit over trajectories. The problem is that it depends on x(0), but we have discussed to normalize and look at the worst case (max eigenvalue of P from a Riccati equation)

 

Insight  from examples and benchmarks

 

·       Second order example : Bicycle MPC  with given velocity and curvature

·       Fourth order example to illustrate a more difficult case of training and evaluation

·       How much is gained by using a projection layer compared to a simple NN?

·       How many layers are needed compared to projected LQR (one layer)  ?

 

 

Summary - What is our conclusion so far?

 

This was a real bad idea or NN with projection layers are fantastic for approximating MPC control laws!

 

Future work

 

·       Parametric MPC problems where the system/model is changing over time e.g LPV MPC,

 

o   http://cse.lab.imtlucca.it/~bemporad/teaching/mpc/imt/2-ltv_nl_mpc.pdf

o   https://users.isy.liu.se/rt/johanl/2012_TAC_LPVMPC.pdf

 

·       Can we instead learn NN to approximate the MPC cost to go function  (value function)  to find the optimal control law? Related  to reinforcement learning.

 

·       In real MPC the state is measured and hence we  do not need super high precision  in approximating the MPC control low. How could we get this into the training and evaluation? What happens if we evaluate train and with noisy x?

==> CDC 2020 MPC-NET/training_datagen.tex <==
We first discuss the systematic strategy that we propose for the generation of datasets for the MPC problems. Our approach for generating the training and testing data set involves sampling a set of states $\mathcal{S} = \{\mathbf{x}_1\, \hdots, \mathbf{x}_{N_S}\}$ from the feasible region $\mathcal{C}_{\infty}$ described in Section II-B, followed by solving for the optimal control inputs for each $s \in \mathcal{S}$ using OSQP \cite{OSQP}. To sample $\mathcal{C}_{\infty}$ we use the Hit-and-Run sampler which is a Markov chain Monte Carlo method for sampling uniformly from convex shapes \cite{METE20126}.  Essentially, starting from any point in the convex set, the method generates a set of points, $\mathcal{S}$, by walking random distances, $\lambda$, in randomly generated (unit) directions. The steps involved in the Hit-and-Run sampler are detailed in Algorithm \ref{alg:har}. We employ this approach since it ensures that the generated datapoints cover the feasibility region in a reasonably uniform manner \cite{METE20126, Zabinsky2013}. This then ensures that the network has observed training samples that span the entire feasible set on an average, thereby aiding its ability to generalize. Once the training and test inputs are generated, the corresponding training outputs are obtained from using OSQP on to solve the MPC problem.

\begin{algorithm}
\label{alg1}
\caption{Hit-and-Run Sampler}\label{alg:har}
\begin{algorithmic}[1]
\Procedure{Hit-and-Run }{$\mathcal{C}_{\infty}, N_S$}
\State Pick random point $\mathbf{x} \in \mathcal{C}_{\infty} = \{\mathbf{x} \in \mathbb{R}^n \mid \mathbf{C}_x\mathbf{x} \leq \mathbf{d}_x\}$
\State $\mathcal{S} \leftarrow \{\mathbf{x}\}$
\For{$i = 1, \hdots, N_S-1$}
\State $\lambda_i \leftarrow \infty$
\State Generate random unit direction $\mathbf{d}_i$
\For {$(\mathbf{c},d)$ in $(\mathbf{C}_x,\mathbf{d}_x)$}
\State $\lambda \leftarrow \displaystyle\frac{d-\mathbf{c}\cdot \mathbf{x}}{\mathbf{c}\cdot\mathbf{d}_i}$
\If {$\lambda > 0$} \Comment{To ensure right direction}
\State $\lambda_i \leftarrow \text{min}(\lambda_i, \lambda)$
\EndIf
\EndFor
\State $\lambda_i \leftarrow \text{drawn from }\mathbb{U}[0,\lambda_i)$
\State $\mathbf{x} \leftarrow \mathbf{x} + \lambda_i\mathbf{d}_i$
\State $\mathcal{S} \leftarrow \mathcal{S} \cup \{\mathbf{x}\}$
\EndFor
\State \textbf{return} $\mathcal{S}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

We then use a supervised learning method to train the networks on a data set $\mathcal{D} = \{(\mathbf{x}_i,\mathbf{u}_i^*)\}$ of input-output pairs. 
During the training, we learn for the network parameters by minimizing a loss function $L(\theta)$ with respect to $\mathbf{\theta}$. 
%The most commonly used/default loss function for regression analysis is the Mean Square Error (MSE) \cite{mseloss}
In this work, we consider mean-square error as the loss function:
\begin{equation}
    L(\theta) = \frac{1}{N}\sum_{i=0}^{N-1}(n(\mathbf{x}_i,\mathbf{\theta}) - \mathbf{u}_i^*)^2.
\label{eq:mse_loss}
\end{equation}
%which is also what has been used in this work.
In order to increase the training speed, we split the data into smaller subsets (mini-batches) and compute the MSE-loss (\ref{eq:mse_loss}) for each batch. We then use the gradient descent-based \textit{Adam} optimizer \cite{adam} to backpropagate the loss and update the parameters $\mathbf{\theta}$ following each batch. Once all the mini-batches have been iterated over, one training epoch is completed. We train the networks for as many epochs required to reach convergence.


%\\\\
%For sampling $C_{\infty}$ we propose the Hit-and-Run sampler in Algorithm %\ref{alg:har}, a Markov chain Monte Carlo method for sampling uniformly from %convex shapes.
%\\\\
%For generating training and testing data sets, we propose a random walk approach %in which we start by sampling the feasible region $C_{\infty}$ hit-and-run sampler 
%\\\\
%To generate the training and testing data sets, we start by first sampling a %subset of $N_S$ states from the feasible region $C_{\infty}$ using the hit-and-run sampler in Algorithm \ref{alg:har}. We then proceed using OSQP \cite{osqp} to solve for the optimal control inputs for each state. 
%\\\\



==> story.tex <==
STORY LINE

 

We consider MPC of linear systems with linear constraint and quadratic cost function …

 

Questions: Use notation from the OSQP paper or the book? I suggest the OSQP notation

 

We use the standard MPC theory for feasibility and stability, ref book by Bemporad & co

 

We use OSQP for solving the MPC  to generate training data.

 

Why is it a good idea to store the solution for all x rather than running real time optimization? The vehicle industry is used to look up table control  and it is easy to evaluate/certify  by massive simulations

 

 

We have to understand  how the MPC control law u=\mu(x) looks like as a function of x

 

In order of simplicity

 

·       LQR u=-Lx

·       LQR with projection on the constraints

·       Explicit MPC

·       QP with linear constraints, take from OSQP paper that the solution for fixed active sets given by a set of linear equations. It is even more clear from the attached book chapter main.pdf (section 2.2). The challenge is that the active constraints are changing as a function of $x$ ( explicit MPC).

·       We can calculate the gradient of \mu(x) w.r.t. x using CVXPY: We expect the gradient to be constant in area where the control law is linear, and jump when we move between active constraint. Nice with a plot for the 2 state example. Plot mu(x) its derivative from dense gridding.

 

We have to understand  data generation for u=\mu(x), i.e. how should we sample x to obtain “optimal” information about the function =\mu(x) to be used for supervised learning?

 

·       LQR is easy. Just pick n linearly independent values of x and solve a linear equation

·       Explicit MPC is more difficult: Pick n linearly independent values of x in each subset where the control law is constant and solve  linear equations

·       Random sampling using hit and run. This is a good idea for covering a higher dimension set by random sampling

·       Should we use trajectories or not to for learning data?

·       Supervised sampling  where one needs new samples of where the fit is bad. Here we may use ideas from Gaussian Processes etc as I wrote

 

 

Given all this information other authors has proposed to use NN with ReLU and projection layers.

 

·       We have combined PyTorch and CVXPY to an easy environment for training and evaluation

·       There are guidelines in how many layers one needs for a given state dimension

·       There are some evidence that the projection layers are need, but we are not sure

·       How do we evaluate the learned NN? Here we propose  to measure the fit over trajectories. The problem is that it depends on x(0), but we have discussed to normalize and look at the worst case (max eigenvalue of P from a Riccati equation)

 

Insight  from examples and benchmarks

 

·       Second order example : Bicycle MPC  with given velocity and curvature

·       Fourth order example to illustrate a more difficult case of training and evaluation

·       How much is gained by using a projection layer compared to a simple NN?

·       How many layers are needed compared to projected LQR (one layer)  ?

 

 

Summary - What is our conclusion so far?

 

This was a real bad idea or NN with projection layers are fantastic for approximating MPC control laws!

 

Future work

 

·       Parametric MPC problems where the system/model is changing over time e.g LPV MPC,

 

o   http://cse.lab.imtlucca.it/~bemporad/teaching/mpc/imt/2-ltv_nl_mpc.pdf

o   https://users.isy.liu.se/rt/johanl/2012_TAC_LPVMPC.pdf

 

·       Can we instead learn NN to approximate the MPC cost to go function  (value function)  to find the optimal control law? Related  to reinforcement learning.

 

·       In real MPC the state is measured and hence we  do not need super high precision  in approximating the MPC control low. How could we get this into the training and evaluation? What happens if we evaluate train and with noisy x?
